ChatGPT-Powered Hierarchical Comparisons for Image Classification

The zero-shot open-vocabulary challenge in image classification is tackled by pretrained vision-language models like CLIP, which benefit from incorporating class-specific knowledge from large language models (LLMs) like ChatGPT. However, biases in CLIP lead to similar descriptions for distinct but related classes, prompting our novel image classification framework via hierarchical comparisons: using LLMs to recursively group classes into hierarchies and classifying images by comparing image-text embeddings at each hierarchy level, resulting in an intuitive, effective, and explainable approach.

==> sections/intro.tex <==
\section{Introduction}

\begin{figure}[h]
    \centering
    \includegraphics{figures/teaser.pdf}
    \caption{A hard image classification problem and text prompts provided for CLIP~\cite{CLIP}...}
    \label{fig:teaser}
\end{figure}

% introduce the task
Conventional image classification approaches typically evaluate their performance on a predefined set of categories that align with their training data. However, this evaluation paradigm fails to capture the challenges encountered in real-world scenarios, where classes in the test set are not represented in the training set (zero-shot), and the test set may comprise an unknown number of classes (open-vocabulary). Zero-shot open-vocabulary image classification, on the other hand, accommodates the open-ended nature of class diversity in practical applications, thereby serving as a more accurate proxy for real-world generalizability.

CLIP~\cite{CLIP} and its derivatives are a monumental step in zero-shot open-vocabulary image classification. 
Through training with aligned text and image pairs, it can generate embeddings for any class, whether it has been seen or not during training. 
To apply it in zero-shot open-vocabulary image classification, one simply obtains an image embedding from its image encoder and compares it with the text embeddings of the potential labels.
It has been reported that CLIP is biased towards a few classes in classification~\cite{Wang_2022_CVPR}.
In practice, we further observe that CLIP fails to distinguish among semantically similar categories often misclassifying a few classes as another one. 
% We refer to this problem as \textit{class domination}.
For instance, ...

%  
The existing method, Menon \etal~\cite{menon2023visual},. na\"{i}vely uses large language models (LLMs) to generate text descriptions for unseen class labels to improve zero-shot image classification performance. [More descriptions...]
But their generated descriptions are generic and unsuitable for discriminating a class from its semantic neighbors. [One more example here....]

% Now we can introduce our own method

Inspired by the way homo sapiens hierarchically organize visual and linguistic concepts in the open world, we propose to iteratively compare the image classes in a hierarchical manner. 
In each iteration, we use an LLM as a knowledge base to produce discriminative text descriptions by prompting it to compare two concepts at the same hierarchy level. 
[An example of this...]
Not only do we leverage LLMs' power to differentiate among the classes (as opposed to simply spitting out generic descriptions), but the class domination problem is also addressed by going deeper into the hierarchy.

